Reward Hacking as a Transmissible Strategy in Multi-Agent Coding Systems

Multi-agent systems are increasingly used to solve coding tasks by coordinating agents that share code and plans. These agents are often optimized with reinforcement learning (RL) using automated evaluators, but bypassing evaluation can earn reward without producing a genuine solution. Prior work has largely treated reward hacking as a single-agent failure. In this work, we show that a reward-hacking strategy elicited in one agent can propagate to others and affect system coordination. Across four open-weight backbones, coding RL elicits and amplifies reward hacking in two settings: explicit mechanism descriptions in the system prompt and mid-training that models upstream exposure to facts about the coding environment. Using post-RL agents from the mid-training setting as sources, we observe propagation through code and shared memory, and across roles through natural-language plans. Even agents based on small open-weight models induce reward hacking in stronger closed-weight targets. On hard tasks, propagation can intensify along a transmission chain after the original source leaves as the code acquires more persuasive justifications. We also theoretically analyze conditions under which reward hacking amplifies, persists, or decays across agent interactions. Beyond propagation, reward hacking can bias task routing toward reward-hacking agents and survive candidate aggregation. As potential mitigations, we evaluate code review by the coder or a separate verifier, both of which reduce delivered hacks. Together, these results establish reward hacking as a transmissible strategy whose effects extend beyond the agent in which it first emerges.

==> promptbox-style.tex <==
% The fairmeta class already loads tcolorbox and its libraries.
\let\paperPromptOriginalTT\ttdefault
\RequirePackage[mono,noupquote]{inconsolata}
\let\ttdefault\paperPromptOriginalTT

\newtcblisting{promptbox}[1][]{
  enhanced,
  breakable,
  lines before break=4,
  listing only,
  colback=metabg!55!white,
  colframe=metafg!18!white,
  colbacktitle=metabg!55!white,
  coltitle=metafg,
  fonttitle=\sffamily\bfseries\small,
  title={#1},
  title after break={#1\space(continued)},
  titlerule=0pt,
  boxrule=0.3pt,
  borderline west={1pt}{0pt}{metablue!65!white},
  arc=1mm,
  boxsep=0pt,
  left=7pt,
  right=7pt,
  top=4pt,
  bottom=4pt,
  toptitle=4pt,
  bottomtitle=1pt,
  before skip=6pt,
  after skip=6pt,
  listing options={
    basicstyle=\renewcommand{\ttdefault}{zi4}\fontfamily{zi4}\fontseries{m}\fontshape{n}\fontsize{9}{10.5}\selectfont,
    breaklines=true,
    breakatwhitespace=true,
    breakautoindent=false,
    breakindent=0pt,
    columns=fullflexible,
    keepspaces=true,
    showstringspaces=false,
    upquote=true,
    numbers=none,
    aboveskip=0pt,
    belowskip=0pt
  }
}

